Cohomological properties of the quantum shuffle product and application to the construction of quasi-Hopf algebras

For a commutative algebra the shuffle product is a morphism of complexes. We generalize this result to the quantum shuffle product, associated to a class of non-commutative algebras (for example all the Hopf algebras). As a first application we show that the Hochschild-Serre identity is the dual statement of our result. In particular, we extend this identity to Hopf algebras. Secondly, we clarify the construction of a class of quasi-Hopf algebras.

==> fig/comp.tex <==
\begin{picture}(0,0)%
\epsfig{file=ps/comp.ps}%
\end{picture}%
\setlength{\unitlength}{3947sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(240,845)(1388,-801)
\put(1463,-214){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}\special{ps: gsave 0 0 0 setrgbcolor}\small$f$\special{ps: grestore}}}}
\put(1468,-489){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}\special{ps: gsave 0 0 0 setrgbcolor}\small$g$\special{ps: grestore}}}}
\end{picture}


==> fig/moddroi-1.tex <==
\begin{picture}(0,0)%
\epsfig{file=ps/moddroi-1.ps}%
\end{picture}%
\setlength{\unitlength}{3947sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(4688,1814)(901,-1436)
\put(1634,-1378){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}$\varphi_L$}}}
\put(901,-845){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(1035,-845){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(1302,-845){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(1901,-845){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(2035,-845){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(2168,-845){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(1368, 89){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}$\dots$}}}
\put(1634,-511){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}$\dots$}}}
\put(2434, 89){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}$\dots$}}}
\put(2434,-511){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}$\dots$}}}
\put(2835,-845){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(1501,-845){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(1435,-1177){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}$p+2$}}}
\put(2368,-1177){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}$q+2$}}}
\put(4301,-1378){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}$\varphi_R$}}}
\put(3568,-845){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(4234,-845){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(4368,-845){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(4500,-845){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(5101,-845){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(5501,-845){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(5300,-845){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(4901, 89){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}$\dots$}}}
\put(4634,-511){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}$\dots$}}}
\put(3901, 89){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}$\dots$}}}
\put(4901,-845){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(3901,-511){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}$\dots$}}}
\put(3700,-1177){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}$p+2$}}}
\put(4767,-1177){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12}{\rmdefault}{\mddefault}{\updefault}$q+2$}}}
\end{picture}


==> fig/morpsi.tex <==
\begin{picture}(0,0)%
\epsfig{file=ps/morpsi.ps}%
\end{picture}%
\setlength{\unitlength}{0.00083300in}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(1936,1645)(1039,-4036)
\put(1051,-3702){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(1174,-3702){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(1296,-3702){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(1726,-3702){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(1910,-3702){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(2033,-3702){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(2217,-3702){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(1480,-3456){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{\rmdefault}{\mddefault}{\updefault}$\dots$}}}
\put(1358,-4009){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{\rmdefault}{\mddefault}{\updefault}$n+2$}}}
\put(2462,-4009){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{\rmdefault}{\mddefault}{\updefault}$n+2$}}}
\put(1849,-2597){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{\rmdefault}{\mddefault}{\updefault}$\dots$}}}
\put(2585,-3702){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(2769,-3702){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(2892,-3702){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(2364,-3456){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{\rmdefault}{\mddefault}{\updefault}$\dots$}}}
\end{picture}


==> fig/prod.tex <==
\begin{picture}(0,0)%
\epsfig{file=ps/prod.ps}%
\end{picture}%
\setlength{\unitlength}{0.00083300in}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(365,546)(713,-710)
\put(713,-686){\makebox(0,0)[lb]{\smash{\SetFigFont{8}{9.6}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(1013,-686){\makebox(0,0)[lb]{\smash{\SetFigFont{8}{9.6}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\end{picture}


==> fig/psidn.tex <==
\begin{picture}(0,0)%
\epsfig{file=ps/psidn.ps}%
\end{picture}%
\setlength{\unitlength}{0.00083300in}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(5819,1864)(589,-1597)
\put(1019,-1219){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(1298,-1219){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(1507,-1219){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(1995,-1219){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(2135,-1219){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(2274,-1219){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(741,-1219){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(601,-1219){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(810,-1567){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}$n+2$}}}
\put(2413,-452){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}$\egpoi$}}}
\put(4435,-452){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}$\egpoi$}}}
\put(880,-731){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}$\dots$}}}
\put(1716,-731){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}$\dots$}}}
\put(2623,-1219){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(2762,-1219){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(3180,-1219){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(3320,-1219){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(3529,-1219){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(4017,-1219){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(4156,-1219){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(4295,-1219){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(3250, 36){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}$\dots$}}}
\put(2901,-731){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}$\dots$}}}
\put(3738,-731){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}$\dots$}}}
\put(6317,-1219){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(6177,-1219){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(6038,-1219){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(5550,-1219){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(5271,-1219){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(5132,-1219){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(4783,-1219){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(4644,-1219){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(5132, 36){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}$\dots$}}}
\put(5689,-731){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}$\dots$}}}
\put(4923,-731){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}$\dots$}}}
\put(1298, 36){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{13.2}{\rmdefault}{\mddefault}{\updefault}$\dots$}}}
\end{picture}


==> fig/sig-1.tex <==
\begin{picture}(0,0)%
\epsfig{file=ps/sig-1.ps}%
\end{picture}%
\setlength{\unitlength}{0.00083300in}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(451,523)(601,-637)
\put(601,-614){\makebox(0,0)[lb]{\smash{\SetFigFont{8}{9.6}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(983,-614){\makebox(0,0)[lb]{\smash{\SetFigFont{8}{9.6}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\end{picture}


==> fig/sig.tex <==
\begin{picture}(0,0)%
\includegraphics{ps/sig.eps}%
\end{picture}%
\setlength{\unitlength}{3947sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(472,590)(1179,-697)
\put(1269,-661){\makebox(0,0)[rb]{\smash{\SetFigFont{8}{9.6}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\put(1651,-661){\makebox(0,0)[rb]{\smash{\SetFigFont{8}{9.6}{\rmdefault}{\mddefault}{\updefault}\pa}}}
\end{picture}

